A Systematic Procedure for Topological Path Identification with Raw Data Transformation in Electrical Distribution Networks

This paper introduces a systematic approach to address the topological path identification (TPI) problem in power distribution networks. Our approach starts by listing the DSO's raw information coming from several sources. The raw information undergoes a transformation process using a set of transformation functions. This process converts the raw information into well-defined information exploitable by an algorithm. Then a set of hypothetical paths is generated, considering any potential connections between the elements of the power distribution system. This set of hypothetical paths is processed by the algorithm that identifies the hypothetical paths that are compatible with the well-defined information. This procedure operates iteratively, adapting the set of transformation functions based on the result obtained: if the identified paths fail to meet the DSO's expectations, new data is collected, and/or the transformation functions found to be responsible for the discrepancies are modified. The systematic procedure offers practical advantages for DSOs, including improved accuracy in path identification and high adaptability to diverse network configurations, even with incomplete or inaccurate data. Consequently, it emerges as a useful tool for the construction of digital twins of power distribution networks that aligns with DSO expectations.

==> Files/CaseStudy.tex <==
\noindent Despite the generality of the method, this systematic procedure is applied to a real distribution network in Belgium.
Given the raw information, multiple steps are performed to reconstruct the network and identify an approximation of the hypothetical paths set compatible with the well-defined information, denoted as $\hat{\mathcal{H}}^{\mathcal{I}'}$.\\

\noindent This section is structured as follows: Section \ref{cs:input} provides an overview of the information employed and the process through which the raw information is converted into well-defined information using transformation functions. Subsequently, Section \ref{cs:algo} focus on how the algorithm is applied to identify the active and backup paths compatible with the well-defined information.\\

% \subsection{\textcolor{red}{Input/Preliminary steps}} \label{cs:input}
\subsection{Data available} \label{cs:input}
\noindent In this particular case, the set of types it is known and can be listed as:
\begin{align}
     \mathcal{T} = \{ & customer, \; cabinet, \; connection \; board \\
     & transformer, \; open \; switch, \; close \; switch, \nonumber \\
     & pole, \; underground, \; overhead \nonumber
     \}.
\end{align}
% Cabinet: https://electrical-engineering-portal.com/res2/Elements-of-power-distribution-systems.pdf . Page 91, image 3.115
Where elements of type $customer$ represent the end-users or consumers,
$cabinet$ represent the junctions that connect customers to the network,
$transformer$ denote the medium-to-low voltage transformers,
$connection \; board$ are panels after the transformers where all electrical connections are organised,
$open \; switch$ and $close \; switch$ present the elements of type switch and their status, 
$underground$ are cables installed under the ground and $overhead$ is a cable installed above the ground usually supported by elements of type $pole$.
\\
% For the subsets of each type, the number of elements and their location is known. There are a few exceptions concerning certain elements. For instance, for $connection \; board$ only the location is known but not the number, and for $open \; switch \text{ and } close \; switch$ both the number and the location are unknown. For some other elements it is possible that the type is not known, these elements fall under the type $unknown$.\\

\noindent The raw information available to the DSO is listed as follows:
\begin{enumerate}
    \item[$i_1$:] Power distribution networks common design practises.
    \item[$i_2$:] GIS data about the coordinates of the elements.
    \item[$i_3$:] GIS data may be affected by errors.
    \item[$i_4$:] Images showing comparisons between satellite images and GPS locations of elements of type $overhead$, revealing some potential misalignments.
    \item[$i_5$:] Document showing connections of elements of types $cabinet$ and $underground$.
    \item[$i_6$:] Discussion with DSO about the distance between elements of types $cabinet$ and $underground$.
    \item[$i_7$:] Plans showing connections of elements of types $connection \; board$ and $pole$.
    \item[$i_{8}$:] Images showing connections of elements of types $customer$, $cabinet$ and $pole$.
    \item[$i_9$:] Discussion with DSO where they state that switches are close to element of type $cabinet$.
    \item[$i_{10}$:] Discussion with DSO where they state that the status of the switches is unknown.
\end{enumerate}

\noindent \\
The raw information is transformed in well-defined information by the transformation functions as follows:
\begin{enumerate}
    \item[$i'_1$]$= f_1(i_1)$: There is one and only one customer, connection board and transformer in any path.
    
    % \item[$i'_2$]$= f_2(i_1)$: Each element can be repeated at most once in a given path. e.g. the path $p = (..., e_i, ..., e_i, ...)$ is not allowed, with $e_i \in \mathcal{E}$.
    
    \item[$i'_2$]$= f_2(i_1)$: Two consecutive elements of the same set can not follow each other directly. For example, it is not possible to have 2 consecutive elements of a given type $t \in \mathcal{T}$. i.e. the path $p = (..., e_i, e_j, ...)$ is not allowed, with $e_i,e_j \in Subset(\mathcal{E}, t)$

    \item[$i'_3$]$= f_3(i_1)$: Paths can be composed by at most $N$ elements, and the distance from the $customer$ and $transformer$ is at most $D_p$.
    
    \item[$i'_4$]$= f_4(i_1)$: Transformers have limited capacity. A transformer can supply no more than a given number of customers, $M$. 
    
    \item[$i'_5$]$= f_5(i_2, i_3)$: The GPS coordinates for the elements are assumed to be correct.
    
    \item[$i'_6$]$= f_6(i_4)$: The extreme of an element of type $overhead$ is extended to the closest extreme of an element of type $overhead$ if inside a given threshold distance, $D_{oh}$. In this case, $D_{oh}$ is chosen as $1$ meters.
    
    \item[$i'_7$]$= f_7(i_5, i_6)$: Elements of type $cabinet$ are connected to the closest element of type $underground$ if inside a given threshold distance, $D_{cab}$. In this case, $D_{cab}$ is chosen as $2$ meters.
    
    \item[$i'_{8}$]$= f_{8}(i_7)$: The extremes of an element of type $pole$ are extended to the closest element of type $connection \; board$ if inside a given threshold distance, $D_{cb}$. In this case, $D_{cb}$ is chosen as $2$ meters.
    
    % \item[$i'_{9}$]$= f_{9}(i_7)$: Elements of type $connection \; board$ are connected to the closest element of type $pole$ with an $overhead$ line. 
    
    \item[$i'_{9}$]$= f_{9}(i_8)$: Elements of type $customers$ are connected to elements of type $cabinet$ or $pole$. The actual connection type, either $underground$ or $overhead$, to an  element of type $cabinet$ or $pole$, depends on which one is closer. 
    
    \item[$i'_{10}$]$= f_{10}(i_9, i_{10})$: Elements of type $open \; switch$ or $close \; switch$ are identified with a recursive algorithm.
\end{enumerate}
% \textcolor{red}{A (sub)section here to describe relationships and ontologies used in this work?}

\subsection{Algorithm} \label{cs:algo}
The algorithm to reconstruct the network and to identify an approximation of the hypothetical paths set, $\hat{\mathcal{H}}^{\mathcal{I}'}$, is composed of the following steps.\\
% Each step is characterised by some assumptions.

\subsubsection{Overhead lines misalignment}
% The inaccuracies in GPS recordings for the overhead lines can be problematic when their extremities are expected to overlap perfectly but, fail to do so. To tackle this issue, we connect together the overhead lines that are located within a specified threshold distance. \\
% The threshold distance, $D_{oh}$, is chosen to be $1$ meters.\\
Considering the well-defined information $i'_5$ and $i'_6$, the set $\mathcal{L}_{oh}$ is mathematically expressed as follows:
\begin{align}
    \mathcal{L}_{oh} = \{ l \; | \; & Dist(e, n^*)<D_{oh}, \\
    & n^* = Closest\bigl(e, Subset(\mathcal{E},overhead)\bigl), \nonumber \\
    &l.coor = (e.coor, n^*), \, l.type=overhead \nonumber \\
    & \forall e \in Subset(\mathcal{E},overhead) \nonumber \}.
\end{align}

% \begin{algorithm}
% \caption{Connect Underground Lines to Armoires}
% \begin{algorithmic}[1]
%     \REQUIRE set of elements $E$, threshold distance $D_{oh}$
%     % \ENSURE List of pairs $(n^*, m^*)$ representing feasible connections: $L$
    
%     % \STATE $L \longleftarrow \emptyset$
    
%     \FOR{each element $e$ in $Subset(\mathcal{E}, overhead)$}
%         % \STATE Initialize $t$ as \textit{None}
%         % \STATE Initialize $l$ as \textit{None}
%         \STATE $n^* = Closest(e, Subset(\mathcal{E}, overhead))$
%         % \STATE $m^* = Closest(e^{|e|}, Subset(\mathcal{E}, armoire))$
    
%         \IF{ $Dist(e, n^*) < D_{oh}$ and $e \neq n^*$}
%             \STATE $l \longleftarrow (COOR(e), COOR(n^*)^0)$
%             \STATE $t \longleftarrow underground$
%             % \STATE Set the type of $l$ as $t$
%             \STATE  $Subset(\mathcal{E}, overhead) \longleftarrow Subset(\mathcal{E}, overhead)-\{e\}+\{l\}$
%         \ENDIF
%     \ENDFOR
%     % \STATE Substitute $Subset(\mathcal{E}, underground)$ with $L$
%     \RETURN $\mathcal{E}$
% \end{algorithmic}
% \end{algorithm}

\noindent This expression defines the set of elements of type $overhead$, denoted as $\mathcal{L}_{oh}$. These elements meet the criteria that the distance between element $e$ to the coordinate of its closest element of type $overhead$, $n^*$, must be within $D_{oh}$ ($Dist(e, n^*)<D_{oh}$). The overhead line is extended to the closest overhead line extremity found, $(e.coor, n^*)$.
Given this set of underground line, $\mathcal{L}_{oh}$, the elements in $Subset(\mathcal{E},overhead)$ whose extremities were extended are substituted by $\mathcal{L}_{oh}$.\\
This step reduces the $\hat{\mathcal{H}}^{\mathcal{I}'}$ space since it removes some lines of type $overehad$ that must not be considered, therefore it eliminates the hypothetical paths that used those lines, similarly as shown in the example, Fig. \ref{fig:example}.\\


\subsubsection{Underground lines to cabinets}
% The misalignment of cabinets and underground lines due to inaccurate GPS location can create complications when they are anticipated to align seamlessly but do not. To address this issue, we connect the underground lines to the closest cabinet if they are within a certain threshold distance.\\
% The threshold, $D_{cab}$, is chosen to be $2$ meters.\\
% Therefore, the assumptions for this step are:
% \begin{enumerate}
%     \item[$a_1$:] underground lines can be connected to only nodes of the type $cabinet$.
%     \item[$a_2$:] underground lines are connected to the closest cabinet if inside a given threshold distance, $D$; otherwise the lines are not, considered. In this case, $D$ is chosen as $8$ meters.
% \end{enumerate}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.41\textwidth]{Images/under cabinet.png}
%     \includegraphics[width=0.45\textwidth]{Images/under cabinet 2.png}
%     \caption{Left: the lines are connected to the cabinet since their distance is lower than a given distance $D$.\\
%     Right: since the distance is more than the threshold D, the top line cannot be connected to an cabinet and is not considered in the network.}
%     % \label{fig:my_label}
% \end{figure}
Considering the well-defined information $i'_5$ and $i'_7$, the set $\mathcal{L}_{cab}$ is mathematically expressed as follows:
\begin{align}
    \mathcal{L}_{cab} = \{ l \; | & Dist(e, n^*)<D_{cab} \land Dist(e, m^*)<D_{cab}, \\
    & n^* = Closest\bigl(e^0, Subset(\mathcal{E},cabinet)\bigl), \nonumber \\
    & m^* = Closest\bigl(e^{|e|}, Subset(\mathcal{E},cabinet)\bigl), \nonumber \\
    &l.coor = (n^*, e.coor, m^*), \, l.type=underground \nonumber \\
    & \forall e \in Subset(\mathcal{E},underground) \nonumber \}.
\end{align}
This expression defines the set of elements of type $underground$ connected to the elements of type $cabinet$, denoted as $\mathcal{L}_{cab}$. These elements must satisfy the condition that the distances of extremes of the element of $e$ ($e^0$ and $e^{|e|}$) to $n^*$ and $m^*$, where $n^*$ and $m^*$ are the coordinates of the closest elements of type $cabinet$ to respectively the first and last extreme of the element $e$, must be within $D_{cab}$, i.e. $Dist(e, n^*) < D_{cab}$ and $Dist(e, m^*) < D_{cab}$.\\
% The new line is extended to $n^*$ and $m^*$.\\
Given this set of underground line $\mathcal{L}_{cab}$, the previous subset of underground elements, $Subset(\mathcal{E},underground)$, is substituted with the new one, $\mathcal{L}_{cab}$.\\
This step reduces the $\hat{\mathcal{H}}^{\mathcal{I}'}$ space since it removes some lines of type $underground$ that must not be considered, therefore it eliminates the hypothetical paths that used those lines.\\

\subsubsection{Connection boards lines}
% MV/LV substations are facilities used to transform the voltage from medium to low voltage, so that it is possible to supply energy to the customers. These substations are buildings that contain one transformer, for this reason in this work the terms substation and transformer are used interchangeably.\\
% \noindent The absence of connection boards' connection to the grid poses significant issues since there would be not electricity in the grid. To address this situation, we connect the connection boards to the grid by linking them to the closest elements of type $pole$ or $underground$ element.
\noindent Considering the well-defined information $i'_5$ and $i'_{8}$, the set $\mathcal{L}_{cb}$ is mathematically expressed as follows:
\vspace{-\baselineskip}
% \noindent Considering the well-defined information $i'_5$ and $i'_{8}$, the set of underground lines that belongs to connection boards, $\mathcal{L}_{cb \rightarrow ug}$, can be mathematically expressed as follows:
% \begin{align}
%     \mathcal{L}_{cb \rightarrow ug} \! = \! \{ &l \; | \\
%     & Dist(e, n^*)<D_{cb}, \nonumber \\
%     & n^* = Closest(e, n) \; \forall n \in Subset(\mathcal{E},underground), \nonumber \\
%     &l = \bigl(Coor(e), n^*\bigl), Type(l)\!=\!underground \nonumber \\
%     & \forall e \in Subset(\mathcal{E},connection \; board) \nonumber \}.
% \end{align}
% This expression defines the set of underground lines, denoted as $\mathcal{L}_{cb \rightarrow ug}$, that meet the distance criteria $Dist(e, n^*)<D_{cb}$ that indicates that the distance between $e$ and $n^*$ must be within $D_{cb}$. The underground line is extended to the closest connection board found, $(Coor(e), n^*)$.\\

% \noindent Moreover, according to $i'_{9}$, connection boards are also connected to $pole$ elements with an $overhead$ cable.
% \begin{align}
%     \mathcal{L}_{cb \rightarrow oh} = \{ & l \; | \\
%     (&t=underground \land p = n^{*}) \; \lor \nonumber \\ 
%     \bigl( &t=overhead \land p = m^{*} \nonumber \\
%         & \;\;\;\;\;\;\;\;\;\;\;\;\;\; \iff Dist(e, n^{*}) < Dist(e, m^{*}) \bigl), \nonumber \\
%     & n^{*} = Closest(e, n) \; \forall n \in Subset(\mathcal{E}, cabinet), \nonumber \\
%     & m^{*} = Closest(e, m) \; \forall m \in Subset(\mathcal{E}, pole), \nonumber \\
%     & l = ( Coor(e), Coor(p) ), \; Type(l) = t \nonumber \\
%     &\forall e \in Subset(\mathcal{E}, connection \; board) \; \} \nonumber.
% \end{align}
\begin{align}
    \mathcal{L}_{cb} = \{ l \; | \; & Dist(e, n^*)<D_{cb}\\
    & n^{*} = Closest\bigl(e,Subset(\mathcal{E}, pole)\bigl), \nonumber \\
    & l.coor = ( e.coor, n^{*} ), \; l.type = overhead \nonumber \\
    &\forall e \in Subset(\mathcal{E}, connection \; board)\} \nonumber.
\end{align}
The expression defines the set of elements of type $overhead$, $\mathcal{L}_{cb}$, representing connections from connection boards to the closest poles with overhead lines. \\ 
% A connection board line, $l$, connects a connection board to an element of type $pole$ with and $overhead$ line.\\
% \noindent Given the sets of underground lines for the elements of type $connection \; board$, $\mathcal{L}_{cb \rightarrow ug}$ and for the elements of type $cabinet$, $\mathcal{L}_{cab}$, the previous subset of underground elements, $Subset(\mathcal{E},underground)$, is replaced by $\mathcal{L}_{cb \rightarrow ug}$ and $\mathcal{L}_{cab}$.
% Moreover, the overhead lines to the connection board, $\mathcal{L}_{cb \rightarrow pol}$, are added to the set of elements, $Subset(\mathcal{E},overhead)$.\\
% This step reduces the $\hat{\mathcal{H}}^{\mathcal{I}'}$ space by eliminating hypothetical paths that involve connections between connection boards and cabinets to elements that are located far from each other.\\
% \noindent Given the sets of underground lines for the elements of type $connection \; board$, $\mathcal{L}_{cb \rightarrow ug}$ and for the elements of type $cabinet$, $\mathcal{L}_{cab}$, the previous subset of underground elements, $Subset(\mathcal{E},underground)$, is replaced by $\mathcal{L}_{cb \rightarrow ug}$ and $\mathcal{L}_{cab}$.
The overhead lines to the connection board, $\mathcal{L}_{cb}$, are added to the set of elements, $Subset(\mathcal{E},overhead)$.\\
This step reduces the $\hat{\mathcal{H}}^{\mathcal{I}'}$ space by eliminating hypothetical paths that involve connections between connection boards and cabinets to elements that are located far from each other.\\

\subsubsection{Customer connections}
% The absence of customers' connections from their households to the grid poses some issue in having a connected power network. To address this situation, we connect the households to the grid by linking them to the closest elements of type $pole$ or $cabinet$ with an $overhead$ or $underground$ element.
\noindent Considering the well-defined information $i'_5$ and $i'_{9}$, the set $\mathcal{L}_{cus}$ is mathematically expressed as follows:
\begin{align}
    \mathcal{L}_{cus} = \{ l \; | \; 
    & \bigl(t=underground \land p = n^{*} \!\!\! \iff \!\!\! B(e,n^*,m^*)\bigl), \nonumber \\
    & \bigl(t=overhead \land p = m^{*} \!\!\! \iff \!\!\! B(e,m^*,n^*)\bigl), \nonumber \\
    & \; n^{*} = Closest\bigl(e,Subset(\mathcal{E}, cabinet)\bigl), \nonumber \\
    & \; m^{*} = Closest\bigl(e,Subset(\mathcal{E}, pole)\bigl), \nonumber \\
    & \; l.coor = ( e.coor, p ), \, l.type = t \nonumber \\
    & \; \forall e \in Subset(\mathcal{E}, customer) \}.
\end{align}
where $B(e,n^*,m^*)$ is a boolean condition given by:
\[
    B(e,n^*,m^*) = Dist(e,n^*) < Dist(e,m^*)
\]
The expression defines the set of lines, $\mathcal{L}_{cus}$, representing connections from the customers to the main grid. A customer line, $l$, connects a customer to a $cabinet$ with an $underground$ cable or to a $pole$ with $overhead$ cable ($t=underground \lor t=overhead$). The choice between an element of type $cabinet$ and $pole$ is based on the distances between the customer and the closest cabinet $n^{*}$ and pole $m^{*}$ $\bigl( Dist(e, n^{*}) < Dist(e, m^{*})\bigl)$.\\
All the elements of this new set, $\mathcal{L}_{cus}$, are added to $\mathcal{E}$.\\
This step reduces the $\hat{\mathcal{H}}^{\mathcal{I}'}$ space by eliminating hypothetical paths that involve connections between customers and elements that are located far from each other.\\

\subsubsection{Switches locations}
% Distribution feeders often operate radially to ensure a reliable and efficient power supply. The use of open switches allows for this radial operation. However, the specific locations of these open switches within the distribution network are not explicitly specified. \\
% % \begin{figure}[h!]
% %     \centering
% %     \includegraphics[width=0.5\textwidth]{Images/Switch locations.png}
% %     \caption{Switches are located between two substations so that any customer is supplied by one and only one substation.}
% %     % \label{fig:my_label}
% % \end{figure}
% \noindent In the absence of precise information or explicit specifications, switches are found manually looking at the map, according to the well-defined information $i'_8$. The process of manually identifying switches can be considered as an algorithm that involves human intervention. In this framework, a human agent is called to visually inspect the map, with a graphical software, like QGIS, and determine the placement of switches.\\
Distribution feeders often operate radially to ensure a reliable and efficient power supply. The use of open switches allows for this radial operation. However, the specific locations of these open switches within the distribution network are not explicitly specified. \\
\noindent Switches are found with a recursive function, according to the well-defined information $i'_5$ and $i'_{10}$.
This function checks the network to ensure that elements cannot be reached through multiple routes by adding elements of type $open \; switch$ or $close \; switch$ as needed.\\

\noindent The $LocateSwitches()$ function takes as input the set of elements, $\mathcal{E}$, the set of types, $\mathcal{T}$ and it output two sets of elements for  $open \; switch$ and $close \; switch$. This function is defined as follows:
\begin{itemize}
    \item It starts defining the empty sets of elements $\mathcal{V}$, $\mathcal{E}_{os}$, $\mathcal{E}_{cs}$.
    \item It iterates over all elements of $\mathcal{E}$. It finds the neighbours, $e_{next}$:
    \begin{itemize}
        \item if $e_{next}$ is already in $\mathcal{V}$, add an element of type $open \; switch$ to $\mathcal{E}_{os}$;
        \item if the type of the element $e_{next}$ is $cabinet$, add an element of type $close \; switch$ to $\mathcal{E}_{cs}$;
        \item otherwise add $e_{next}$ to $\mathcal{V}$ and keep iterating;
        \item if no $e_{next}$ is available, empty the set $\mathcal{V}$ and start with a new element.
    \end{itemize}
    \item It returns the sets $\mathcal{E}_{os}$ and $\mathcal{E}_{cs}$.
\end{itemize}
The returned sets $\mathcal{E}_{os}$ and  $\mathcal{E}_{cs}$ are added to the set $\mathcal{E}$.\\
This step helps to identify active and backup paths.\\

\subsubsection{Paths identification}
Given the connection between the elements, it is possible to identify the hypothetical paths for all the customers. This is achieved with a recursive function, $IdentifyPaths()$, that starts from a customer and loops until it finds an element of type $transformer$ or the number of iteration is greater, $N$, or the total distance greater than $D_p$ (according to the well-defined information $i'_3 \in \mathcal{I}'$).\\
Such recursive function takes as input the set of elements, $\mathcal{E}$, the set of types, $\mathcal{T}$, and the well-defines information, $\mathcal{I}'$ and it outputs a set of hypothetical paths compatible with the well-defined information, denoted as $\hat{\mathcal{H}}^{\mathcal{I}'}$. This function, $IdentifyPaths()$, can be expressed as:
\begin{align}
    \hat{\mathcal{H}}^{\mathcal{I}'} &= IdentifyPaths(\mathcal{E}, \mathcal{T}, \mathcal{I}') = \\
    &= \{\hat{h}^{\mathcal{I}'} \; | \; Path(c, \mathcal{E}, 0, \{\}), \; \hat{h}^{\mathcal{I}'} \neq \emptyset\, \nonumber \\ 
    & \;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \forall c \in Subset(\mathcal{E}, customer) \}. \nonumber
\end{align}
\noindent where $Path(c, \mathcal{E}, k, V)$ is a helper function that traverses the elements, $\mathcal{E}$, starting from an element of type $customer$, $c$; $k$ is a counter that represents the number of steps already taken in the recursive function, and $V$ is a set of visited elements used to prevent that elements are checked twice.\\

\noindent The helper function $Path(c, \mathcal{E}, k, V)$ is defined as follows:
\begin{itemize}
    \item It starts iterating from any element of type $customer$, $c \in Subset(\mathcal{E}, customer)$.
    \item It finds all elements connected to $c$, and for each of these elements denoted as $e_{next}$:
    \begin{itemize}
        \item if the new element, $e_{next}$ is an element of type $transformer$, stops and return the found path given by the sequence of elements, $V$.
        \item if the counter $k$ is grater than $N$, the total distance greater than $D_p$, or $e_{next}$ is already in $V$, stops and return an empty set, since it did not find a transformer.
        \item otherwise, recursively explore all neighbouring elements by calling the function again with the new parameters, \\$Path(e_{next}, \mathcal{E}, k+1, \{c\})$.
    \end{itemize}
    \item Return the path as the result.
\end{itemize}
\textcolor{white}{.}\\
\vspace{-\baselineskip}

\subsubsection{Diagnostic function}
Following the generation of the subset of hypothetical paths compatible with the well-defined information, denoted as $\hat{\mathcal{H}}^{\mathcal{I}'}$ as output of the algorithm, the final step involves an evaluation of the obtained solution using the $Diagnostic()$ function. The primary role of the $Diagnostic()$ function is to evaluate the solution $\hat{\mathcal{H}}^{\mathcal{I}'}$, and report any issues or discrepancies in the found paths. \\
This function considers the well-defined information: $i'_1$, $i'_2$, $i'_3$, $i'_4$. Some of the possible problems are: some elements are disconnected from the main grid, some customers have no path, paths with inadequate length, rings in the network or too short lines. These represent some issues that need to be addressed.\\
In such cases, the transformation functions responsible for the discrepancies are modified to accommodate these issues, and the execution of the algorithm is repeated. If the revised solution proves to be problem-free, $\hat{\mathcal{H}}^{\mathcal{I}'}$ is then considered solution of the TPI problem.\\

\noindent To illustrate this with an example, after identifying the solution $\hat{\mathcal{H}}^{\mathcal{I}'}$, and running the $Diagnostic()$ function, it may become clear that the number of elements of type $underground$ does not align with requirements. Upon identifying the transformation function responsible for this discrepancy, denoted as $f_7$, it is then modified, resulting in an updated well-defined information:
\begin{enumerate}
    \item[$i'_7$]$= f_7(i_5, i_6)$: Elements of type $cabinet$ are connected to the closest element of type $underground$ if inside a given threshold distance, $D_{cab}$. In this case, $D_{cab}$ is chosen as $4$ meters.
\end{enumerate}
In this example, the distance $D_{cab}$ was increased to consider some discrepancies with the reality.\\
% The $Diagnostic()$ function evaluates the solution's consistency to the specified well-defined information. Adjustments ensure that any deviations are adjusted, ultimately leading to a reliable solution to the TPI problem.

\subsubsection{Identification of active and backup paths}
Given an approximation of the compatible hypothetical paths and the switches elements, it is possible to identify the hypothetical active and backup paths. The set of active hypothetical paths for a particular customer element $c \in Subset(\mathcal{E}, customer)$ can be found with the following mathematical operation:
% \begin{align}                      \hat{\mathcal{H}}^{\mathcal{I}'}_{a,c} = \{ & p \in \hat{\mathcal{H}}^{\mathcal{I}'}_{c} \; |\\
% & \bigl(\nexists \; e \in p : Type(e)=open \; switch \; \land \nonumber \\
% &Type(e)=close \; switch \bigl) \; \lor \nonumber \\
% & Type(e)=close \; switch \; \forall e \in p\}. \nonumber
% \end{align}
\begin{align}                      \hat{\mathcal{H}}^{\mathcal{I}'}_{a,c} = \{ & \hat{h}^{\mathcal{I}'} \!\! \in \hat{\mathcal{H}}^{\mathcal{I}'}_{c} \; | \nexists \; e \in \hat{h}^{\mathcal{I}'} \!\! : e.type=open \; switch \}
\end{align}

\noindent where $\hat{\mathcal{H}}^{\mathcal{I}'}_{a,c}$ denotes the collection of compatible hypothetical active paths of the element customer ($c$). These paths are determined by the condition that there are no elements of type switches (neither open nor close) in each path $p \in \hat{\mathcal{H}}^{\mathcal{I}'}_{c}$,or that the type of all the elements of each path is close switch.\\

\noindent Similarly, the subset of the compatible hypothetical backup paths of a customer $c$, is given by:
% \begin{align}
%     \hat{\mathcal{H}}^{\mathcal{I}'}_{b,c} = \{ p \in \hat{\mathcal{H}}^{\mathcal{I}'}_{c} \; |& \; (\exists \; e \in p : Type(e)=open \; switch \; \lor Type(e)=close \; switch) \; \land \\
%     & Type(e)=close \; switch \; \forall e \in p\}.
% \end{align}
\begin{align}                                 \hat{\mathcal{H}}^{\mathcal{I}'}_{b,c} = \{ & \hat{h}^{\mathcal{I}'} \!\! \in \hat{\mathcal{H}}^{\mathcal{I}'}_{c} \; | \exists \; e \in \hat{h}^{\mathcal{I}'} \!\! : e.type=open \; switch \}
\end{align}
\noindent where $\hat{\mathcal{H}}^{\mathcal{I}'}_{b,c}$ denotes the collection of backup paths of the customer, $c$. These paths are determined by the condition that there exists at least one element in each path of type $open \; switch$.


==> Files/appendices.tex <==
\appendices
\section{Pseudo-algorithms}

\begin{algorithm}
\caption{Connect Underground Lines to Armoires algorithm}
\begin{algorithmic}[1]
    \REQUIRE Set of all elements: $E$
    \REQUIRE Maximum distance threshold: $D$
    % \ENSURE List of pairs $(n^*, m^*)$ representing feasible connections: $L$
    
    \STATE Initialize an empty list $L$
    
    \FOR{each element $e$ in $Subset(\mathcal{E}, underground)$}
        \STATE Initialize $t$ as \textit{None}
        \STATE Initialize $l$ as \textit{None}
        \STATE $n^* = Closest(e^1, Subset(\mathcal{E}, armoire))$
        \STATE $m^* = Closest(e^{|e|}, Subset(\mathcal{E}, armoire))$
    
        \IF{ $Dist(e^1, n^*) < D$ and $Dist(e^{|e|}, m^*) < D$ and $n^* \neq m^*$}
            \STATE Set $l$ as $(COOR(n^*), COOR(m^*))$
            \STATE Set $t$ as $underground$
            \STATE Set the type of $l$ as $t$
            \STATE Append the pair $l$ to the list $L$
        \ENDIF
    \ENDFOR
    \STATE Substitute $Subset(\mathcal{E}, underground)$ with $L$
    \RETURN $\mathcal{E}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Connect customers to main feeder algorithm}
\begin{algorithmic}[1]
    \REQUIRE Set of all elements: $E$
    % \ENSURE List of pairs $(n^*, m^*)$ representing feasible connections: $L$
    
    \STATE Initialize an empty list $L$
    
    \FOR{each element $e$ in $Subset(\mathcal{E}, customer)$}
        \STATE Initialize $t$ as \textit{None}
        \STATE Initialize $l$ as \textit{None}
        \STATE $n^* = Closest(e, Subset(\mathcal{E}, armoire))$
        \STATE $m^* = Closest(e, Subset(\mathcal{E}, pole))$
    
        \IF{ $Dist(e, n^*) < Dist(e, m^*)$}
            \STATE Set $l$ as $(Coor(e), Coor(n^*))$
            \STATE Set $t$ as $armoire$
        \ELSE
            \STATE Set $l$ as $(Coor(e), Coor(m^*))$
            \STATE Set $t$ as $pole$
        \ENDIF
        \STATE set the type of $l$ as $t$
        \STATE Append the pair $l$ to the list $L$
    \ENDFOR
    
    \STATE Add $L$ to $\mathcal{E}$
    \RETURN $\mathcal{E}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Find switches location algorithm}
\begin{algorithmic}[1]
    \REQUIRE Set of all elements: $E$
    % \ENSURE List of pairs $(n^*, m^*)$ representing feasible connections: $L$

    \STATE Initialise $\mathcal{S}$ as $None$
    \STATE $\mathcal{S} = HumanInspection()$
    
    \STATE Add $\mathcal{S}$ to $\mathcal{E}$
    \RETURN $\mathcal{E}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Generate graph algorithm}
\begin{algorithmic}[1]
    \REQUIRE Set of all elements: $\mathcal{E}$
    % \ENSURE List of pairs $(n^*, m^*)$ representing feasible connections: $L$

    \STATE TO BE DEFINED (not the focus of this work?)
    
    % \STATE add $\mathcal{E}'$ to $\mathcal{E}$
    \RETURN $\mathcal{G}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Iterative helper function paths}
\begin{algorithmic}[1]
    \REQUIRE Graph: $\mathcal{G}$
    \REQUIRE Customer element: $e$
    \REQUIRE Set of all elements: $\mathcal{E}$
    \REQUIRE Steps Counter: $k$
    \REQUIRE Set of all already visited elements: $V$
    
    \STATE Set $N$ as the maximum number of steps
    \STATE $e_{nexts}$ = FindConnectedElements($\mathcal{G}$, $e$)

    \FOR{each element $e_{next}$ in $e_{nexts}$}
        \IF{$Type(e_{next}) == transformer$}
            \RETURN $V$
        \ELSIF{$e_{next} \in V$ or $k > N$}
            \RETURN $NONE$
        \ELSE
            \STATE Add $e$ to $V$
            \STATE k = k + 1
            \STATE $Paths(\mathcal{G}, e_{next}, \mathcal{E}, k, V)$
        \ENDIF
    \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Find compatible hypothetical paths}
\begin{algorithmic}[1]
    \REQUIRE Set of all elements: $\mathcal{E}$
    \REQUIRE Set of all information: $\mathcal{I}$
    \REQUIRE Set of all assumptions: $\mathcal{A}$
    
    \FOR{each element $e$ in $Subset(\mathcal{E}, customer)$}
        \STATE Initialise $h$ as $None$

        h = $Paths(\mathcal{G}, e, \mathcal{E}, 0, \{\})$
        \IF{h is not $None$}
            \STATE Add $h$ to $\hat{\mathcal{H}}^{(\mathcal{I},\mathcal{A})}$
        \ENDIF
    \ENDFOR

    \RETURN $\hat{\mathcal{H}}^{(\mathcal{I},\mathcal{A})}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Main algorithm}
\label{algo:meth}
\begin{algorithmic}[1]
    \REQUIRE set of elements $\mathcal{E}$
    \REQUIRE set of types $\mathcal{T}$
    \REQUIRE set of information $\mathcal{I}$
    \REQUIRE set of assumptions $\mathcal{A}$
    % \ENSURE The sum of the first $n$ positive integers
    % \STATE $sum \gets 0$
    \STATE $\mathcal{E} = ConnectUndergroundLines2Armoires(\mathcal{E})$
    \STATE $\mathcal{E} = ConnectCustomers2Feeder(\mathcal{E})$
    \STATE $\mathcal{E} = LocateSwitches()$
    \STATE $\mathcal{G} = GenerateGraph(\mathcal{E})$
    \STATE $\hat{\mathcal{H}}^{(\mathcal{I},\mathcal{A})} = 
    FindPaths(\mathcal{G},\mathcal{E},\mathcal{I},\mathcal{A})$
\end{algorithmic}
\end{algorithm}
